Attackers reveal their arsenal: An investigation of adversarial techniques in CTI reports

Context: Cybersecurity vendors often publish cyber threat intelligence (CTI) reports, referring to the written artifacts on technical and forensic analysis of the techniques used by the malware in APT attacks. Objective: The goal of this research is to inform cybersecurity practitioners about how adversaries form cyberattacks through an analysis of adversarial techniques documented in cyberthreat intelligence reports. Dataset: We use 594 adversarial techniques cataloged in MITRE ATT\&CK. We systematically construct a set of 667 CTI reports that MITRE ATT\&CK used as citations in the descriptions of the cataloged adversarial techniques. Methodology: We analyze the frequency and trend of adversarial techniques, followed by a qualitative analysis of the implementation of techniques. Next, we perform association rule mining to identify pairs of techniques recurring in APT attacks. We then perform qualitative analysis to identify the underlying relations among the techniques in the recurring pairs. Findings: The set of 667 CTI reports documents 10,370 techniques in total, and we identify 19 prevalent techniques accounting for 37.3\% of documented techniques. We also identify 425 statistically significant recurring pairs and seven types of relations among the techniques in these pairs. The top three among the seven relationships suggest that techniques used by the malware inter-relate with one another in terms of (a) abusing or affecting the same system assets, (b) executing in sequences, and (c) overlapping in their implementations. Overall, the study quantifies how adversaries leverage techniques through malware in APT attacks based on publicly reported documents. We advocate organizations prioritize their defense against the identified prevalent techniques and actively hunt for potential malicious intrusion based on the identified pairs of techniques.

==> garbage/cover.tex <==
Dear Editor,

We wish to submit an original research article entitled “Attackers reveal their arsenal: An investigation of adversarial techniques in CTI reports” for consideration.

We confirm that this work is original and has not been published elsewhere, nor is it currently under consideration for publication elsewhere.

In this paper, I/we report on / show that _______. This is significant because __________.

In this paper, we perform an investigation on the adversarial techniques used by malware used in advanced persistent threat attacks. We 

We believe that this manuscript is appropriate for publication by [journal name] because it… [specific reference to the journal’s Aims & Scope]. __________.

[Please explain in your own words the significance and novelty of the work, the problem that is being addressed, and why the manuscript belongs in this journal. Do not simply insert your abstract into your cover letter! Briefly describe the research you are reporting in your paper, why it is important, and why you think the readership of the journal would be interested in it.]

We have no conflicts of interest to disclose. Thank you for your consideration of this manuscript.

Sincerely,
Md Rayhanur Rahman

==> garbage/garbage.tex <==
% multi-stage cyberattacks
% - threats for big companies
% - hard to detect
% - mean time to detect is very large
% - 6 months
% - the better we know about this, the better the defend can be

% why CTI reports?
% - provide context of large scale cyberattacks
% - malware as a unique combination of attack techniques (software vector).
% - very big companies are compromised. provides a view on why big organizations are failing to secure
% - provides a lessons for organizations about future attacks
% - they are written by profession security vendors
% - provides enough details 
% - collectively sends us a message about how incidents happened and what should we do to not repeat them
% - providea a view on attackers toolset
% - Some publicly available databases record cyber security incidents, but these databases are heavily biased towards incidents that require public disclosure and large-scale incidents at major organizations that are reported by the media [3]. Therefore, many open questions exist about the statistical properties of cyber security incidents and their implications for the organization of security response.

% what has been done so far
% - primary focus is still into two things: IoC extraction, TTPs extraction, and linking TTPs to system logs
% - these work helps us in identifying high and low level indicators, also identiying possible alerts as APTs. they solve the alert fatigure problem, they solve the manual CTI report parsing problem.
% - however, these work does these under the hood. Based on the existing data, they make decisions. and SIEM/SOC people use them. But, there is a need for informing how TTPs work in these attacks, and how to gain a deeper understanding, 
% - however, there is little research on what are collectively in this reports and what could be the generalized form of learning
% - focus on pyramid of pain. IoCs are short term. attackers can change this. But ttps are long term. A machine learning framework for investigating data breaches based on semantic analysis of adversary’s attack patterns in threat intelligence repositories
% - Understanding the behaviour is important so that people can learn about threat lanscxape. and how these behaviours are linked to each other
% - These traditional tools are indeed crucial for protecting the network premises; however, they do not provide two pivotal features, making the security analyst blind to APT attacks: (a) understanding the causal relationship between diferent system events [44]; and (b) piecing together attack artifacts over a long period of time [3]. Most current threat hunting approaches also operate only on partial views of cyber attacks such as detection based on known IOCs, e.g., malware hash values, IP addresses of C&C, domain names owned/controlled by the attackers, ile names used by the APTs [23, 58]; using heuristics [63], e.g., checking if a ile appears to be a variant of known malware; or by using local behavior analysis [46]. The irst method (known IOCs) can pinpoint exact known malware samples, but it misses mutated malware versions [70, 71]. The other two techniques may be able to detect mutated malware but often trigger a high rate of (costly) false positives [66]. Other threat hunting mechanisms include network system behavior analysis tools (e.g., [76]) and ile system behavior analysis tools (e.g., [74]) which are based on detecting anomalies from the learned system normal behavior. However, they also generate an unmanageable number of false positives [9, 56], unless tuned with higher thresholds, which on the other hand, increase the probabilities of missing attacks.
% - Public reporting on cyber threats has been growing throughout the past decade. However, there has yet to be a comprehensive analysis of the information disclosed in such reports and the trends and patterns hidden within them. An analysis of publicly available reporting on cyber threat actors, the techniques they employ for operations, and the sectors of critical infrastructure at risk of an attack, can provide the cybersecurity community with a stronger understanding of the publicly available information at their disposal (as it relates to critical infrastructure cybersecurity). The findings derived from such an analysis can be used to enhance both cyber practitioners’ and academics’ understanding of the content and trends present in government cyber reporting while also identifying gaps in the public information sharing landscape. The goal of this study is to analyze publicly available reporting on cyber threats and develop an understanding of the changes in reporting, throughout the past decade.

% shown an example CTI reports
% - reflect the multi-stage nature
% - reflect prevalent techniques
% - reflect ttps are abstract, but could be different in implementation
% - reflect the combination

% The purpose of this research is to discover the knowledge in public cyber attack databases, organizing them in a structured way to be used in the improvement of the threat hunting process.

% what's the goal?
% - understand the nature of multistage cyberattacks
% - understand the structure of cyberattacks
% - how attacks are pieced together by combining TTPs
% - characterization of multi-stage cyberattacks through the lense of TTPs
% - characterization of adversarial actions forming multi stage cyberattacks 
% - prevalent actions, prevalent procedures, what combinations are prevalent
% - characterization of how adversarues form multi-stage cyberattacks through the usage of TTPs
% - The goal of this research is to aid practitioners in understanding the 


% Why do we need to find prevalent techniques?
% - provides a view to the threat landscape
% - emerging TTPs
% - a context for defenders for optimizing their defense
% - what attack vectors are prevalent
% - policies, antivirus features
% - The purpose of threat modeling is to provide defenders with a systematic analysis of what controls or defenses need to be included, given the nature of the system, the probable attacker's profile, the most likely attack vectors, and the assets most desired by an attacker. Threat modeling answers questions like “Where am I most vulnerable to attack?”, “What are the most relevant threats?”, and “What do I need to do to safeguard against these threats?”.

% Why do we need to analyze procedure
% - TTPs are abstract in nature
% - but procedures are implementation. There are various ways a ttp can be executed
% - characterize the TTPs
% - characterize the implementation, attack vectors, abuse of system components
% - can aid us forseeing what different ways these can be implemented in future
% - heuristics for anti virus

% why relations
% - nature of the links among the TTPs
% - role of the TTP in context of an attack
% - high level understanding of alert correlation
% - key TTPs to defend
% - threat hunting hypothesis
% - heuristics

% contributions
% - every steps can be a contribution


% relation types
% - assets
% - - security implication: assets that have two vectors or vectors that can be abused by two techniques. If two techniques work on a same asset, then asset can be protected so that further attack cannnot happen. If two techniques work on similar types of asset, then it can indicates different possible attack paths to a technique. All similar assets have to be protected. 
% - overlap
% -- 


% TODO
% \begin{enumerate}
%     \item define why we used pearson's phi. because we tried to model attacker's opportunistic view
%     \item In the discussion section, emphasize theoretical actionability. Plot and score techniques by $(frequency \times trend) \times (pagerank\_centrality \times diversity)$. this can be called as $prevalence-coverage$. 
%     \item   from an attackers pov, this plot indicates the  weak points of an organization. from a defenders point of view, these are common weak points attack can come through
%     \item If a technique is related to various types of relationships, the technique is a threat from different types and vectors.
%     \item Build two datasets, and illustrate the practical application of the theory: CTI reports and APTGen. Build a node2vec model. Then search for TTPs by $similarity$ of TTPs recursively in $n$ depths. CTI-reports for a random search, APTGen for a sequential search. 
% \end{enumerate}


% % dump from introduction

% % Existing studies on CTI reports in the literature focus on primarily the following two: (a) automatically extracting malware indicators (e.g., malware hash, IP address) and adversarial techniques (e.g., phishing, exploiting vulnerability) from written descriptions of cyberattack~\cite{liao_acing_2016, husari_ttpdrill_2017, satvat_extractor_2021, Gao2021EnablingEC}; and (b) mapping intrusion alert logs to adversarial techniques to detect ongoing multi-stage attacks~\cite{milajerdiHOLMESRealTimeAPT2019, weiDeepHunterGraphNeural2021a, mahmoudAPTHunterDetectingAdvanced2022}. In practice, endpoint detection and response system (EDR) and security event identification and management (SEIM) tools focus on identifying low-level malware indicators. However, low-level indicators are helpful for a short period and often lack context. For example, an attacker can change the IP address of its botnets. The IP address also does not reflect the context, such as not providing information on if it is used as an ex-filtration destination or to deliver malware. 




% % Example 1 shows an excerpt from an actual CTI report describing a cyberattack incident in 2022 where the attack originated from phishing emails. Upon clicking the email attachment, malicious content is executed in the victim system, and the vulnerability is exploited. The example informs about a list of techniques used, shown in italics: phishing, exploiting vulnerabilities, and downloading malware. The example also shows how combining techniques play a role in the attack. For example, \textit{running} an embedded object, is followed by \textit{downloading} malware, where the object came from a \textit{phishing} attachment. The example demonstrates how to infect a system with malware by combining \textit{phishing} and \textit{downloading} techniques. Overall, practitioners need to utilize the information provided in CTI reports, which can contribute to defending from APT attacks. 

% % The pyramid of pain~\cite{pyramidOfPain}, a conceptual model of thwarting adversaries, emphasizes that, instead of low-level indicators, responding to adversarial techniques is the most effective strategy to prevent cyberattacks. 

% % However, to the best of our knowledge, we find little research on deriving an understanding of the phenomenon: \textit{how the adversarial techniques collectively construct APT attacks} from CTI reports. 

% % instead of focusing on lower levels of relatedness. For example, instead of finding that a particular IP address is always matched with a particular malware hash, our study focuses more on the pattern: malware is downloaded from a C2 address. Practitioners can implement the patterns into EDR and SIEM. They can also utilize those in forensic investigations.

% % \section{Introduction}
% % We can pitch the contribution like this:
% % \begin{enumerate}
% %     \item CTI reports contain lots of knowledge
% %     \item Define and describe both CTI and CTI reports
% %     \item The knowledge is hard to generalizable, and provides an aspect of attack for only a few specific cases like large-scale data breach, apt attacks, etc
% %     \item so the dataset provides a lot of bias; however, still, they provide knowledge
% %     \item eventually this understanding can enable practitioners to understand the structure of cyberattacks through the lens of MITRE ATT\&CK techniques
% %     \item there is nlp and ml work on extracting techniques... but we need to think of in further depth, and there is little work identified. 
% %     \item so we analyze the TTPs in three dimensions: (a) how prevalent, (b) how implemented, (c) how they are interrelated
% %     \item the understanding can lead us to practical threat hunting hypothesis constructions. so we validate our findings in the APTGen synthetic dataset
% %     \item use the motivation and example from the proposal
% % motivational points: alert fatigue, 
% % \end{enumerate}

% % \begin{scriptsize}
% % \begin{longtable}{lp{10cm}}
%     % \toprule
    
%     % \multicolumn{2}{c}{\textbf{TA0001: Initial Access}} \\ \midrule
%     % \multirow{4}{*}{T1566.001: Spearphishing attachment} & \textbf{Attachment types:} Document, archives, URLs, fake installers, shortcut files, malicious binaries and scripts, compiled HTML, HTML applications \\ 
%     % {} & \textbf{Attachment properties:} password-protected, hidden macro, content, scripts, executables, exploits \\ 
%     % {} & \textbf{Prior behavior:} sent from legitimate but compromised account \\ 
%     % {} & \textbf{Follow-on behavior:} Deliver malware, reconnaissance, harvest credentials \\ \midrule

%     % \multicolumn{2}{c}{\textbf{TA0002: Execution}} \\ \midrule
%     % \multirow{4}{*}{T1059.003: Windows Command Shell} & \textbf{OS functionality:} cmd.exe, rundll32.exe, shell commands \\ 
%     % {} & \textbf{Malicious tools executed:} batch scripts, HTML applications, wscript, visual basic scripts, javascripts, portable executables, lua scripts, command-line tools \\
%     % {} & \textbf{Prior behavior:} remote connection, reverse shell \\
%     % {} & \textbf{Associated behavior:} download malware, cryptomining, disable security tool, change password, collection, setup beacons, persistence, windows management instrumentation, post-intrusion cleanup, scan for files, set registry, destroy volume shadow copy, disable recovery, change file permission, reconnaissance, create scheduled task, macro running shell commands, sql running shell commands, executable hidden in shortcuts, execution from IRC channel, in-memory execution \\ \midrule

%     % \multirow{4}{*}{T1059.001: Powershell} & \textbf{OS functionality:} Powershell, Powershell commands \\
%     % {} & \textbf{Malicious tools executed:} batch and Powershell scripts, portable executables \\
%     % {} & \textbf{Prior behavior:} Remote connection, reverse shell \\
%     % {} & \textbf{Associated behavior:} privilege escalation, credential harvesting, download, discovery, reconnaissance, de-obfuscate, lateral movement, create task, exfiltration, collection, persistence, indicator removal, delete volume shadow copy, maintain c2 connection, disable services, add exception to anti-virus, install shim database, pass-the-hash, in-memory, macro execution, spearphishing, Powershell is itself injected with shellcode \\ \midrule
    
%     % \multirow{5}{*}{T1204.002: Malicious File} & \textbf{User action:} Open document, execute scripts, enable macro/content \\
%     % {} & \textbf{Malicious file executed:} Documents, fake installers, fake antivirus, storage applications \\
%     % {} & \textbf{Malicious file properties:} Hidden macro and contents, steganography \\
%     % {} & \textbf{Prior behavior:} Phishing, compromised account \\
%     % {} & \textbf{Follow-on behavior:} download second-stage malware, drive by target, reconnaissance, malware deployment \\ \midrule

%     % \multirow{2}{*}{T1106: Native API} & \textbf{API functionality:} Obtain user agent, sandbox check, registry access, create process, process memory allocation, process thread, remote procedural call, HTTP API, named pipe, DNS, file operations, cryptomining \\
%     % {} & \textbf{Associated behavior:} Process injection, account management, running commands without shell, privilege escalation, indicator removal, collection, obfuscation, corrupt system object \\ \midrule

%     % \multicolumn{2}{c}{TA0003: Persistence} \\ \midrule
%     % \multirow{3}{*}{T1547.001: Registry Run Keys} & \textbf{OS component:} Registry run key, startup folder \\ 
%     % {} & \textbf{Follow-on behavior:} Mimic legitimate application, change software configuration \\
%     % {} & \textbf{Persisting tool:} Malware, backdoor, scripts, file-stealers, downloaders, lnk files, visual basic and Powershell scripts, discovery, dynamic link libraries, malware dropper, malware configuration files \\ \midrule

%     % \multicolumn{2}{c}{TA0005: Defense evasion} \\ \midrule
%     % \multirow{2}{*}{T1027: Obfuscated Files or Information} & \textbf{Approach:} encode, encrypt, compress, password protect, string manipulation, byte order manipulation, steganography, source code obfuscation, API hashing, junk instruction \\
%     % {} & \textbf{Files or information:} source code, command, string, shellcode, function name, variable name, macro, API name, dll name, command line arguments, malware, scripts, documents, email attachments, dynamic link libraries, headers, configurations, installer, plugins, tools, images, payload, remote command-and-control domain, url, exfiltrated files, network packets, filesystem, registry keys, encryption keys, system logs \\ \midrule

%     % \multirow{2}{*}{T1070.004: File Deletion} & \textbf{File types:} malicious executables, decompressed data, installers, registry keys, scheduled task, configuration files, log files, system files, local files, rival malware, interfering files \\
%     % {} & \textbf{When:} Post-installation, post-execution, post-exfiltration \\ \midrule

%     % \multirow{3}{*}{T1140: Deobfuscate/Decode Files or Information} & \textbf{Approach:} decode, decrypt, decompress, steganography, re-assemble, password-protect \\ 
%     % {} & \textbf{Files and information:} payload, command-and-control address, network packets, achieve, scripts, malware, dll, images, library, executables, shellcode, string, exploit, source code, function, API calls, email attachments, macro, credentials, cryptomining keys, command-and-control server credentials, configuration files, driver files \\
%     % {} & \textbf{Follow-on behavior:} Malware deployment, in-memory execution \\ \midrule

%     % \multicolumn{2}{c}{TA0007: Discovery} \\ \midrule
%     % \multirow{7}{*}{T1082: System Information Discovery} & \textbf{System information:} Operating system, processor, memory, disk, display, installed applications, patches and hotfixes, compilers and libraries \\ 
%     % {} & \textbf{User information:} user demography, activity, role, privilege, login status, language, uptime, location, keyboard layout \\
%     % {} & \textbf{System security information:} antivirus, virtual machines, debugger, and sandbox check \\
%     % {} & \textbf{API} systeminfo, fsutil, getlogicaladdress, ioreg, ver, vssadmin \\
%     % {} & \textbf{System component:} Registry, Windows management instrumentation \\
%     % {} & \textbf{Prior behavior:} Phishing \\
%     % {} & \textbf{Follow-on behavior:} Collect filesystem content, register with command-and-control \\ \midrule

%     % \multirow{5}{*}{T1083: File and Directory Discovery} & \textbf{File types:} document, image, key, achieves, drivers, media, environment variables, dynamic link libraries, configuration files, executables, calendar, plugin, crypto-miner, source-code \\
%     % {} & \textbf{File locations:} desktop, program files, home, tmp, browser, recent, system directories, mail, profile, startup, IM, appdata, wallet, backup, .net, mobile app, call, contact, SMS, USB \\
%     % {} & \textbf{Information:} whether malware is downloaded and installed, previous infections, presence of sandbox and debuggers, file permissions and privileges \\ 
%     % {} & \textbf{Prior behavior:} Phishing, macro execution \\
%     % {} & \textbf{Associated behavior:} Search files by extension, name, date, type, keywords \\ \midrule

%     % \multirow{5}{*}{T1057: Process Discovery} & \textbf{Process information:} list of running process, process details, virtual machine check, sandbox check, security software check, permission, privilege \\
%     % {} & \textbf{Process category:} browser, compiler, banking apps, venv, CLR, MSBuild, ADFS, cryptominer, MS Identity \\
%     % {} & \textbf{Associated behavior:} Search process by name, keyword, uptime \\
%     % {} & \textbf{Follow-on behavior:} kill process, kill rival malware \\
%     % {} & \textbf{OS API and features:} tasklist, ps, Windows management instrumentation \\ \midrule

%     % \multirow{2}{*}{T1016: System Network Configuration Discovery} & \textbf{Information:} IP, MAC, DNS, Subnet, gateway, routing \\
%     % {} & \textbf{API:} ipconfig, ifconfig, net stat, nbstat, tracert, arp \\ \midrule

%     % \multirow{2}{*}{T1033: System Owner/User Discovery} & \textbf{User information:} Logged-in status, permission, privilege, group membership, uptime \\
%     % {} & \textbf{API and OS features:} whoami, systeminfo, Windows management instrumentation \\
%     % {} & \textbf{Associated behavior:} Internal reconnaissance \\ \midrule
    
%     % \multicolumn{2}{c}{TA0011: Command and control} \\ \midrule
%     % \multirow{5}{*}{T1105: Ingress Tool Transfer} & \textbf{Tools:} Second stage malware, first stage downloader \\ 
%     % {} & \textbf{Protocols:} Intel AMT, certutils, curl, wget, dget, sql, FTP, HTTP/S, DNS, SCP, WinInet \\ 
%     % {} & \textbf{Associated behavior:} download, transfer, upload, drop, push, deploy, install, write \\
%     % {} & \textbf{Prior behavior:} Stage in public repositories such as github, sendspace, dropbox, file-sharing sites, AWS, Onedrive, downloader came from initial access, phishing, drive by target, macros, after document being opened, scheduled task, psexec \\
%     % {} & \textbf{Follow-on behavior:} Update/upgrade malware, webshell installation, in-memory execution, store in the system log folder \\ \midrule

%     % \multirow{5}{*}{T1071.001: Web Protocols} & \textbf{Protocol:} HTTP/HTTPS, webdav, websocket, Graph API, WinInet, custom protocols \\
%     % {} & \textbf{Tools:} curl, get, Command-and-control frameworks \\
%     % {} & \textbf{Abused asset:} Browsers \\
%     % {} & \textbf{Associated behavior:} Download payload, transfer files, send/receive botnet commands, obfuscation, exfiltration, send initial beacon, identify c2 server, conceal C2 traffic, act as a web server \\ 
%     % {} & \textbf{Associated information repositories:} PasteBin, MS Exchange Server, Dropbox, Telegram \\ \midrule

%     % \multirow{2}{*}{T1071.004: DNS} & \textbf{Associated behavior:} Dynamic DNS, DNS tunneling, hide command-and-control traffic \\
%     % {} & \textbf{DNS records:} A, AAA, OPT, TXT \\ \midrule

%     % \multicolumn{2}{c}{TA0010: Exfiltration} \\ \midrule
%     % \multirow{3}{*}{T1041 Exfiltration Over C2 Channel} & \textbf{Collected information:} Credentials, system information, user information, sensitive files, documents, screenshots \\ 
%     % {} & \textbf{Protocols:} HTTP/S, DNS, Mail, \\
%     % {} & \textbf{Services:} Dropbox, ADFS server, MS Exchange, MS Outlook \\
%     % {} & \textbf{Tools:} Webshell, file stealer \\ 
    
    
%     % \bottomrule 
%     % \caption{How techniques are implemented}
%     % \label{tab:procedureCodes}
% % \end{longtable}
% % \end{scriptsize}

% \subsubsection{Identified axial codes} Below we report the identified axial codes. 
% \begin{enumerate}
%     \item Affected object 544 refers to the system assets impacted by a technique. For example, in case of \textit{T1547.001 Registry Run Keys} technique, the modified registry key is an affected object.
%     \item Context 263 refers to the preceding event or condition of a technique. For example, in case of \textit{T1566.001: Spearphishing attachment} technique, phishing mails are often sent from compromised accounts. Hence, compromised account is a context for this technique.
%     \item Intent 219 refers to the succeeding behavior of a technique. For example, in case of \textit{T1071.001: Web protocols}, downloading malware is the intent because, using the protocol, adversary can download malware into victim system.
     
% \end{enumerate}

% \subsubsection{TA0001: Initial access} T1566.001: Spearphishing attachment is the only prevalent technique in the initial access tactic. We observe that adversaries primarily send document files (i.e., word, spreadsheet, pdf) to victim users. These documents may contain hidden macro, executable contents, or exploit codes which would be executed if the user open the document. Adversaries also send password-protected archive files containing fake installers of legitimate programs - which victim users could install into their system. We observe that adversaries primarily use phishing technique to deliver malware into victim system. 

% \subsubsection{TA0002: Execution} We find four techniques in the execution tactic. In this tactic, adversaries primarily abuse the following: native shell command functionality built-in with the operating system: Windows command shell and Powershell. We observe, these two shell commands are used for subsequent malicious tasks such as downloading malware, information collection, modifying system components, and post-compromise cleanup. Adversaries also use Windows command shell and Powershell with in-memory execution. Such execution results in file-less execution so that malware scanners cannot find the malicious file in the file-system. We also observe the abuse of native API functionalities by the adversaries, primarily for process manipulation and system information collection. The aforementioned three execution techniques are performed by adversaries - however, \textit{T1204.002: Malicious file} technique relies on user execution. The technique happens in the context of \textit{T1566.001: Spearphishing attachment} technique, where the victim user has to open a document, and enable the hidden content for execution. We also observe the use of steganography, where adversaries send image files apparently looking benign, however, the image files contains malicious executables. 

% \subsubsection{TA0003: Persistence} T1547.001: Registry Run Keys is the only prevalent technique in this tactic, and the technique affect the Windows registry run keys. We observe that, adversaries primarily aim to run the malicious operation in the background, and automatically launch while boot. Hence, they abuse the registry run key to make malicious start run in the background while system boot. Moreover, we also observe that, adversaries rename their malware to commonly known background tasks such as software updater, antivirus scanner, Windows services so that victim users do not identify them as suspicious process. 

% \subsubsection{TA0005: Defense evasion} We find three techniques in the execution tactic. Adversaries primarily use \textit{T1027: Obfuscation of files/information} techniques to (a) encrypt, encode, compress the command-and-control communication and malware files, and (b) to obfuscate the variables, values, function calls, statements of the source code and scripts so that the content of the source code is not analyzable. Adversaries also obfuscate the collected data before exfiltration. However, the obfuscated files and data has to be restored to the usable state before use, and adversaries use \textit{T1140: De-obfuscation of file/information} technique in this case. While obfuscation and de-obfuscation techniques help in bypassing defense during an ongoing attack - we observe adversaries use \textit{T1070.004: File Deletion} technique. Using the technique, adversaries deletes all the malware footprints after malware deployment, execution, and exfiltration. 

% \subsubsection{TA0007: Discovery} We find five prevalent techniques in the discovery tactic. Overall, the techniques identifies five types of information about the target system: (a) system, (b) files, (c) running process, (d) network configuration, and (e) user account information. The techniques aids adversaries in performing internal reconnaissance and exfiltrating sensitive, and confidential information. We also observe, adversaries abuse the native operating system APIs and shell commands for obtaining the information. We observe that personal and business-related documents, and running applications are the most affected objects in this tactic. 

% \subsubsection{TA0011: Command-and-control, and TA0010: Exfiltration} We find four techniques in the command-and-control (C2) tactics: (a) \textit{T1105: Ingress Tool Transfer}, (b) \textit{1071.001 Web Protocols}, (c) \textit{1071.004 DNS}, and (d) \textit{T1041 Exfiltration Over C2 Channel}. We observe that the primary actions adversaries perform using the three techniques are to (a) download or deploy malware, (b) communicate with remote adversaries (C2), and (c) exfiltration. Further, we observe that adversary uses native operating system and networking protocols, and services to maintain communication with C2. Finally, we observe that, adversaries often use third party information repositories, and cloud storage (such as Github, Dropbox) as a middle-man for communication between victim system and proxy.




% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % \begin{table}[]
% %     \centering
% %     \footnotesize
    
% %     \begin{tabular}{lp{12cm}}
% %     \toprule
% %     \textbf{Tactic}      & \textbf{Techniques}                                                      \\ \midrule
% %     Reconnaissance &
% %       T1595.002: Vulnerability Scanning, T1589.001: Credentials, T1591.002: Business Relationships, T1593.001: Social Media \\
% %     Resource development & T1608.001: Upload Malware, T1587.001: Malware                            \\
% %     Initial access       & T1190: Exploit Public-Facing Application,                                \\
% %     Discovery            & T1016.001: Internet Connection Discovery, T1482: Domain Trust Discovery, \\
% %     Defense evasion &
% %       T1497.003: Time Based Evasion, T1070: Indicator Removal, T1134: Access Token Manipulation, T1055.004: Asynchronous Procedure Call, T1620: Reflective Code Loading, T1078.004: Cloud Accounts, T1480.001: Environmental Keying \\
% %     Persistence          & T1133: External Remote Services, T1547.012: Print Processors             \\
% %     Lateral movement     & T1021.005: VNC                                                           \\
% %     Collection           & T1213: Data from Information Repositories                                \\ 
% %     Command and control  & T1572: Protocol Tunneling                                               \\ \bottomrule
% %     \end{tabular}%
% % \caption{The emerging techniques}
% % \label{tab:emergingTechniques}
% % \end{table}

% % \begin{table}[]
% %     \centering
% %     \footnotesize

% %     \begin{tabular}{lllr}
% %     \toprule
% %      \textbf{Technique Id} & \textbf{Technique Name} & \textbf{Tactic} & \textbf{\% Reports}      \\
% %     \midrule
% %      T1190     & Exploit Public-Facing Application  & Initial-access       & 4.95  \\
% %      T1497.003 & Time Based Evasion                 & Defense-evasion      & 4.65  \\
% %      T1133     & External Remote Services           & Persistence          & 4.35  \\
% %      T1070     & Indicator Removal                  & Defense-evasion      & 2.55  \\
% %      T1572     & Protocol Tunneling                 & Command-and-control  & 2.40   \\
% %      T1608.001 & Upload Malware                     & Resource-development & 2.10  \\
% %      T1587.001 & Malware                            & Resource-development & 1.95  \\
% %      T1134     & Access Token Manipulation          & Defense-evasion      & 1.65  \\
% %      T1021.005 & VNC                                & Lateral-movement     & 1.35  \\
% %      T1016.001 & Internet Connection Discovery      & Discovery            & 1.35  \\
% %      T1595.002 & Vulnerability Scanning             & Reconnaissance       & 1.35  \\
% %      T1482     & Domain Trust Discovery             & Discovery            & 1.20   \\
% %      T1055.004 & Asynchronous Procedure Call        & Defense-evasion      & 1.20   \\
% %      T1620     & Reflective Code Loading            & Defense-evasion      & 1.05  \\
% %      T1213     & Data from Information Repositories & Collection           & 1.05  \\
% %      T1589.001 & Credentials                        & Reconnaissance       & 0.90  \\
% %      T1078.004 & Cloud Accounts                     & Defense-evasion      & 0.90  \\
% %      T1480.001 & Environmental Keying               & Defense-evasion      & 0.75 \\
% %      T1547.012 & Print Processors                   & Persistence          & 0.45 \\
% %      T1591.002 & Business Relationships             & Reconnaissance       & 0.45 \\
% %      T1593.001 & Social Media                       & Reconnaissance       & 0.45 \\
% %     \bottomrule
% %     \end{tabular}
    
% %     \caption{The emerging techniques}
% %     \label{tab:emergingTechniques}
% % \end{table}

% % \subsection{The emerging techniques}
% % Table~\ref{tab:emergingTechniques} shows the 21 emerging techniques identified from the prevalence matrix. These techniques are of low frequency but are expected to be of high frequency. We discuss our observations on the emerging techniques below:

% % \begin{enumerate}
% %     \item We observe two techniques related to gaining initial entry to a system via exploiting vulnerabilities (\textit{T1190}, \textit{T1595.002}). Despite attackers actively seeking to exploit vulnerabilities of applications, exploiting the vulnerability (\textit{T1190}) is much less frequent than phishing (\textit{T1566.001}). We have rather observed the exploitation of vulnerabilities in \textit{privilege escalation}, \textit{lateral movement}, \textit{and persistence} tactics more than in the \textit{initial access} tactic. A related observation is that we find two techniques where the information related to social media footprint (\textit{T1593.001}) and business relationships (\textit{T1591.002}) among organizations are being abused. Another related technique with social engineering vectors is hosting malware in lookalike sites \textit{T1608.001}. These techniques also correlate with phishing because phishing campaigns often lead victims to apparently safe domains hosted by malware. \textbf{Overall, we can speculate that, for APT actors, abusing social engineering vectors is more prevalent than exploiting a public-facing application for initial access.}

% %     \item We observe seven techniques from \textit{defense-evasion} tactics, suggesting that \textbf{adversaries introduce novel techniques primarily to bypass defense}. These techniques utilize low-level system features and information to avoid malware scanners. For example, adversaries can use environment variables as crypto-graphic keys (\textit{T1480.001}) or load the payload directly to RAM without creating a file in the system (\textit{T1620}). File-based scanners and detectors may fall short of identifying these techniques. For example, a detection system would search \textit{key} or \textit{payload} files in the system but would not find anything and be capable of detecting the techniques. 

% %     \item We observe attackers abuse applications with remote login capabilities, such as the following techniques: \textit{T1133}, \textit{T1021.005}, and \textit{T1078.004}. Often, users install these applications on their desktops, such as protocols for remote login (VNC, RDP, SSH) and cloud applications (Dropbox, Google Drive). If the credentials are compromised, then these applications provide full system access. On the other hand, cloud applications run in the background - hence, an adversary can reconfigure the installed cloud application to exfiltrate documents to adversary-controlled storage locations automatically. \textbf{We speculate that, with the adoption of work-from-home and storing files in the cloud, desktop computers are increasingly running background applications with remote execution and file transfer capabilities - which reflects the emerging techniques of the past five years. }
    
% % \end{enumerate}

% % \begin{scriptsize}
% % \begin{longtable}{lp{14cm}}
% %     \toprule
    
% %     \multicolumn{2}{c}{\textbf{TA0001: Initial Access | T1566.001: Spearphishing attachment}} \\ \midrule
% %     Malicious object & Attachments: Documents (94), archives (14), compiled HTML application (4), links (2), shortcuts (2), fake installers and executables (2) \\
% %     % Intent & Deliver malware (51), harvest credentials (1), reconnaissance (1) \\
% %     % Context & Password-protected (6), hidden macro, and content (6), exploits (4), sent from compromised account (2) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1059.003: Windows Command Shell}} \\ \midrule
% %     System abuse & Use of cmd.exe, command-line-interface, commands, operating system shell, rundll32.exe (256), Windows management instrumentation (WMI) (1) \\
% %     % Intent & Download and deploy malware (12), self cleanup (10), collection and discovery (4), persistence (4), set scheduled task (4), set Registry (3), disable security tools (2), scan for files (2), disable recovery (2), reconnaissance (2), change password (1), change file permission (1), Encrypt (1) \\
% %     % Context & Remote execution (51), macro running command shell, SQL running command shell, shortcuts, internet relay chat channel, in-memory execution (12) \\
% %     Malicious object & Scripts: batch, HTA, wscript, vbs, js, PE, lua (57) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1059.001: PowerShell}} \\ \midrule
% %     System abuse & Powershell, Powershell tool, Powershell commands (143), create task (2), add exception to antivirus (1), pass the hash (1), WMI (1) \\
% %     % Intent & Download malware (28), discovery, reconnaissance, collection (8), persistence, set registry key and keyloggers (6), credential harvest (5), lateral movement (5), process injection (3), de-obfuscate (3), exfiltration (2), privilege escalation (1), cleanup (1), disable recovery (1), disable service (1), install shim database (1) \\
% %     % Context & In-memory (8), remote connection (3), phishing and macro execution (3) \\
% %     Malicious object & Scripts: Powershell, batch, portable executables (11) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1204.002: Malicious File}} \\ \midrule
% %     Action & User open or execution (132), enable macro/content (20) \\
% %     % Context & phishing (80), steganography (3), compromised account (1) \\ 
% %     Malicious object & Weaponized document (21), fake installer, anti virus, and storage (12) \\
% %     % Intent & subsequent download, drive by target, reconnaissance, malware loader activation, malware installation (9) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1106: Native API }} \\ \midrule
% %     System abuse & Windows API (110), API for process manipulation (77), API for system information collection (27), API for file operation (11), API for networking: HTTP, DNS, named pipe (9), Linux API (3), crypto-mining API (2), API for remote procedural call (1) \\
% %     % Intent & process injection (5), account management (4), privilege escalation (3), indicator removal (3), collection (1), obfuscation (1), corrupt object (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0003: Persistence | T1547.001: Registry Run Keys}} \\ \midrule
% %     Affected object & Registry run key (163), System autostart folder, app data folder (71) \\ 
% %     Malicious object & Malware, backdoor, scripts, file-stealers, downloaders, lnk files, visual basic and Powershell scripts, discovery, dynamic link libraries, dropper, configuration files (39) \\
% %     % Intent & Mimicking legitimate applications and updaters (6), modify software configuration (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0005: Defense evasion | T1027: Obfuscation of files/information}} \\ \midrule
% %     Action & Encode, encrypt, compress, password protect, string manipulation, byte order manipulation, steganography, source code obfuscation, API hashing, junk instruction (344) \\
% %     Malicious object & Source code, functions, variables, strings (143), malware files (108), command-and-control (C2) communication files (61) \\
% %     Affected object & Collected data (13), system files (2), secret (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0005: Defense evasion | T1070.004: File Deletion}} \\ \midrule
% %     Action & Post compromise cleanup (111) \\
% %     Malicious object & malware footprint (111) \\
% %     Affected object & local files (81) \\
% %     % Context &  Post-installation and persistence (17), post-execution, privilege escalation (14), post-exfiltration (11), invoked by batch script, scheduled task, macro (5) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0005: Defense evasion | T1140: De-obfuscation}} \\ \midrule
% %     Action & Decode, decrypt, decompress, steganography, re-assemble, password-protect (235) \\
% %     Malicious object & Source code (69), malware (60), C2 communication (57), malware configuration (14) \\
% %     % Context & In-memory deployment of malware (8) \\
% %     Affected object & Documents (3), secrets (3), system files (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1082: System Information Discovery}} \\ \midrule
% %     Information & System information: OS, hardware, patches, upgrades (577), User information: demography, location, activity (44), presence of sandbox, debugger, and antivirus (3), C2, malware installation information (3), installed application information (2) \\
% %     System abuse & systeminfo, reg query, fsutil, getlogicaladdress, ioreg, ver, vssadmin, wmi (38) \\
% %     % Context & Phishing (1) \\
% %     % Intent & Collection (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1083: File and Directory Discovery}} \\ \midrule
% %     Affected object & File location: desktop, program files, home, tmp, browser, recent, system directories, mail, profile, startup, IM, appdata, wallet, backup, .net, mobile app, call, contact, SMS, USB (47), malware installation (6), presence of sandbox, debugger, and antivirus (6), file properties: time, permission, privilege (2), file type: document, image, key, achieves, drivers, media, environment variables, dynamic link libraries, configuration files, executables, calendar files, plugin, cryptocurrency miners, source-code (58) \\
% %     Action & Search files (18) \\
% %     % Context & Phishing (1) \\ 
% %     % Intent & File deletion (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1057 Process Discovery}} \\ \midrule
% %     Information & Process metadata: list of running process (179), process metadata: filename, privilege, permission, uptime, port, execution parameters, modules, creation info, environment variables, integrity (13), security information: check for sandbox and security software (6), rival malware (3) \\
% %     System abuse & OS API: tasklist, ps, wmi, Win32API (35) \\
% %     Affected object & process category: browser, compiler, banking apps, venv, CLR, MSBuild, ADFS, cryptocurrency miner, MS Identity (13) \\
% %     Action & search process (11) \\
% %     % Intent & kill process (2), discovery (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1016 System Network Configuration Discovery}} \\ \midrule
% %     Information & Basic network info: IP, MAC, DNS, subnet, gateway, routing (224) \\
% %     System abuse & Command: ipconfig, ifconfig, net, nbstat, tracert (64) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1033 System Owner/User Discovery}} \\ \midrule
% %     Information & user metadata: username, owner, privilege, groups, security identifier (156), user activity inactive, logged-in, query user (28) \\
% %     System abuse &  whomai, WMI, systeminfo, Win32 API (28) \\
% %     % Intent & reconnaissance (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0011: Command and control | T1105: Ingress Tool Transfer}} \\ \midrule
% %     Action & Get malware/tools: download, transfer, upload, drop, push, deploy, install, write (377), update and upgrade malware and tools (5) \\
% %     Malicious object & second stage malware (160), first stage downloader (2) \\
% %     % Context & Information repository as a malware source: Github, Sendspace, Dropbox, file-sharing sites, AWS, Onedrive (6), downloader came from initial access, phishing, drive by target, macros, after document being opened (6), In-memory (4), Task, psexec (2), webshell (1) \\
% %     System abuse & Intel AMT, certutils, curl, wget, dget, sql, FTP, HTTP/S, DNS, SCP, WinInet (9) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0011: Command and control | T1071.001 Web Protocols}} \\ \midrule
% %     System abuse & Use HTTP/HTTPs (291), Protocols: webdav, websocket, Graph API, WinInet (4), custom http header (3), Commands: wget, curl (2), custom protocol (1) \\ 
% %     % Intent & Exfiltration (7), send initial beacon, identify C2 server (2), conceal C2 traffic (1) \\
% %     % Context & encrypted payload (3), Third party information repository: PasteBin, MS Exchange Server, Dropbox, Telegram (3), webserver (1) \\
% %     Malicious object & C2 frameworks (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0011: Command and control | T1071.004 DNS}} \\ \midrule
% %     System abuse & DNS (44), DNS tunnelling (10), DNS records: AAA, TXT, A, OPT (6), dynanic DNS (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0010: Exfiltration | T1041 Exfiltration Over C2 Channel}} \\ \midrule
% %     Affected object & Data and files exfiltration (86) \\
% %     Information & Collected information: credentials, network information, hostname, username, specific files of interest, documents, screenshots (38) \\
% %     System abuse & Protocol: HTTP/S, DropBox API, DNS, Mail, ADFS server, Exchange web service, outlook (22) \\
% %     Malicious object & Webshell, file stealer (3) \\ 
% %     \bottomrule \\ 
% %     \caption{How techniques are implemented}
% %     \label{tab:procedureCodes}
% % \end{longtable}
% % \end{scriptsize}


% % We identify the number of prevalent and emerging techniques are small portions of the total number of cataloged techniques.  According to the criteria discussed in Section~\ref{rq1Methodology}: the count of prevalent techniques is 18 (3\%). Also, the count of emerging techniques is 21 (3.5\%). We discuss these techniques in Section~\ref{rq1:prevalentTechniques}.

% % We call a technique \textit{emerging} if the technique is in \textit{the top-left} corner because these techniques are infrequent but are expected to be more frequent in the future. 

% \begin{table}[]
% \centering
% \scriptsize
% \begin{tabular}{p{4cm}rp{10cm}}
% \toprule
% \textbf{Category}                & \textbf{Count} & \textbf{Techniques}              \\ \midrule
% Secondary infection              & 160            & T1105: Ingress Tool   Transfer   \\
% Social engineering       & 87 & T1204.002: Malicious File, T1082: System Information   Discovery, T1105: Ingress Tool Transfer                 \\
% Remote and   reverse shell & 54 & T1059.003: Windows Command Shell, T1059.001: PowerShell                                                        \\
% In-memory   execution      & 22 & T1059.003: Windows Command Shell, T1059.001: PowerShell,   T1140: De-obfuscation, T1105: Ingress Tool Transfer \\
% Post-installation                & 17             & T1070.004: File Deletion         \\
% Post-execution                   & 14             & T1070.004: File Deletion         \\
% Post-exfiltration                & 11             & T1070.004: File Deletion         \\
% Run from   external applications & 2              & T1059.003: Windows Command Shell \\
% Primary infection                & 2              & T1105: Ingress Tool Transfer     \\
% Run without shell                & 1              & T1106: Native API          \\ \bottomrule     
% \end{tabular}%
% \caption{Identified codes in the context category}
% \label{tab:axialContext}
% \end{table}

% % \begin{scriptsize}
% % \begin{longtable}{lp{14cm}}
% %     \toprule
    
% %     \multicolumn{2}{c}{\textbf{TA0001: Initial Access | T1566.001: Spearphishing attachment}} \\ \midrule
% %     Malicious object & Attachments: Documents (94), archives (14), compiled HTML application (4), links (2), shortcuts (2), fake installers and executables (2) \\
% %     % Intent & Deliver malware (51), harvest credentials (1), reconnaissance (1) \\
% %     % Context & Password-protected (6), hidden macro, and content (6), exploits (4), sent from compromised account (2) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1059.003: Windows Command Shell}} \\ \midrule
% %     System abuse & Use of cmd.exe, command-line-interface, commands, operating system shell, rundll32.exe (256), Windows management instrumentation (WMI) (1) \\
% %     % Intent & Download and deploy malware (12), self cleanup (10), collection and discovery (4), persistence (4), set scheduled task (4), set Registry (3), disable security tools (2), scan for files (2), disable recovery (2), reconnaissance (2), change password (1), change file permission (1), Encrypt (1) \\
% %     % Context & Remote execution (51), macro running command shell, SQL running command shell, shortcuts, internet relay chat channel, in-memory execution (12) \\
% %     Malicious object & Scripts: batch, HTA, wscript, vbs, js, PE, lua (57) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1059.001: PowerShell}} \\ \midrule
% %     System abuse & Powershell, Powershell tool, Powershell commands (143), create task (2), add exception to antivirus (1), pass the hash (1), WMI (1) \\
% %     % Intent & Download malware (28), discovery, reconnaissance, collection (8), persistence, set registry key and keyloggers (6), credential harvest (5), lateral movement (5), process injection (3), de-obfuscate (3), exfiltration (2), privilege escalation (1), cleanup (1), disable recovery (1), disable service (1), install shim database (1) \\
% %     % Context & In-memory (8), remote connection (3), phishing and macro execution (3) \\
% %     Malicious object & Scripts: Powershell, batch, portable executables (11) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1204.002: Malicious File}} \\ \midrule
% %     Action & User open or execution (132), enable macro/content (20) \\
% %     % Context & phishing (80), steganography (3), compromised account (1) \\ 
% %     Malicious object & Weaponized document (21), fake installer, anti virus, and storage (12) \\
% %     % Intent & subsequent download, drive by target, reconnaissance, malware loader activation, malware installation (9) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0002: Execution | T1106: Native API }} \\ \midrule
% %     System abuse & Windows API (110), API for process manipulation (77), API for system information collection (27), API for file operation (11), API for networking: HTTP, DNS, named pipe (9), Linux API (3), crypto-mining API (2), API for remote procedural call (1) \\
% %     % Intent & process injection (5), account management (4), privilege escalation (3), indicator removal (3), collection (1), obfuscation (1), corrupt object (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0003: Persistence | T1547.001: Registry Run Keys}} \\ \midrule
% %     Affected object & Registry run key (163), System autostart folder, app data folder (71) \\ 
% %     Malicious object & Malware, backdoor, scripts, file-stealers, downloaders, lnk files, visual basic and Powershell scripts, discovery, dynamic link libraries, dropper, configuration files (39) \\
% %     % Intent & Mimicking legitimate applications and updaters (6), modify software configuration (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0005: Defense evasion | T1027: Obfuscation of files/information}} \\ \midrule
% %     Action & Encode, encrypt, compress, password protect, string manipulation, byte order manipulation, steganography, source code obfuscation, API hashing, junk instruction (344) \\
% %     Malicious object & Source code, functions, variables, strings (143), malware files (108), command-and-control (C2) communication files (61) \\
% %     Affected object & Collected data (13), system files (2), secret (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0005: Defense evasion | T1070.004: File Deletion}} \\ \midrule
% %     Action & Post compromise cleanup (111) \\
% %     Malicious object & malware footprint (111) \\
% %     Affected object & local files (81) \\
% %     % Context &  Post-installation and persistence (17), post-execution, privilege escalation (14), post-exfiltration (11), invoked by batch script, scheduled task, macro (5) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0005: Defense evasion | T1140: De-obfuscation}} \\ \midrule
% %     Action & Decode, decrypt, decompress, steganography, re-assemble, password-protect (235) \\
% %     Malicious object & Source code (69), malware (60), C2 communication (57), malware configuration (14) \\
% %     % Context & In-memory deployment of malware (8) \\
% %     Affected object & Documents (3), secrets (3), system files (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1082: System Information Discovery}} \\ \midrule
% %     Information & System information: OS, hardware, patches, upgrades (577), User information: demography, location, activity (44), presence of sandbox, debugger, and antivirus (3), C2, malware installation information (3), installed application information (2) \\
% %     System abuse & systeminfo, reg query, fsutil, getlogicaladdress, ioreg, ver, vssadmin, wmi (38) \\
% %     % Context & Phishing (1) \\
% %     % Intent & Collection (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1083: File and Directory Discovery}} \\ \midrule
% %     Affected object & File location: desktop, program files, home, tmp, browser, recent, system directories, mail, profile, startup, IM, appdata, wallet, backup, .net, mobile app, call, contact, SMS, USB (47), malware installation (6), presence of sandbox, debugger, and antivirus (6), file properties: time, permission, privilege (2), file type: document, image, key, achieves, drivers, media, environment variables, dynamic link libraries, configuration files, executables, calendar files, plugin, cryptocurrency miners, source-code (58) \\
% %     Action & Search files (18) \\
% %     % Context & Phishing (1) \\ 
% %     % Intent & File deletion (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1057 Process Discovery}} \\ \midrule
% %     Information & Process metadata: list of running process (179), process metadata: filename, privilege, permission, uptime, port, execution parameters, modules, creation info, environment variables, integrity (13), security information: check for sandbox and security software (6), rival malware (3) \\
% %     System abuse & OS API: tasklist, ps, wmi, Win32API (35) \\
% %     Affected object & process category: browser, compiler, banking apps, venv, CLR, MSBuild, ADFS, cryptocurrency miner, MS Identity (13) \\
% %     Action & search process (11) \\
% %     % Intent & kill process (2), discovery (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1016 System Network Configuration Discovery}} \\ \midrule
% %     Information & Basic network info: IP, MAC, DNS, subnet, gateway, routing (224) \\
% %     System abuse & Command: ipconfig, ifconfig, net, nbstat, tracert (64) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0007: Discovery | T1033 System Owner/User Discovery}} \\ \midrule
% %     Information & user metadata: username, owner, privilege, groups, security identifier (156), user activity inactive, logged-in, query user (28) \\
% %     System abuse &  whomai, WMI, systeminfo, Win32 API (28) \\
% %     % Intent & reconnaissance (1) \\ 
% %     \midrule

% %     \multicolumn{2}{c}{\textbf{TA0011: Command and control | T1105: Ingress Tool Transfer}} \\ \midrule
% %     Action & Get malware/tools: download, transfer, upload, drop, push, deploy, install, write (377), update and upgrade malware and tools (5) \\
% %     Malicious object & second stage malware (160), first stage downloader (2) \\
% %     % Context & Information repository as a malware source: Github, Sendspace, Dropbox, file-sharing sites, AWS, Onedrive (6), downloader came from initial access, phishing, drive by target, macros, after document being opened (6), In-memory (4), Task, psexec (2), webshell (1) \\
% %     System abuse & Intel AMT, certutils, curl, wget, dget, sql, FTP, HTTP/S, DNS, SCP, WinInet (9) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0011: Command and control | T1071.001 Web Protocols}} \\ \midrule
% %     System abuse & Use HTTP/HTTPs (291), Protocols: webdav, websocket, Graph API, WinInet (4), custom http header (3), Commands: wget, curl (2), custom protocol (1) \\ 
% %     % Intent & Exfiltration (7), send initial beacon, identify C2 server (2), conceal C2 traffic (1) \\
% %     % Context & encrypted payload (3), Third party information repository: PasteBin, MS Exchange Server, Dropbox, Telegram (3), webserver (1) \\
% %     Malicious object & C2 frameworks (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0011: Command and control | T1071.004 DNS}} \\ \midrule
% %     System abuse & DNS (44), DNS tunnelling (10), DNS records: AAA, TXT, A, OPT (6), dynanic DNS (1) \\ \midrule

% %     \multicolumn{2}{c}{\textbf{TA0010: Exfiltration | T1041 Exfiltration Over C2 Channel}} \\ \midrule
% %     Affected object & Data and files exfiltration (86) \\
% %     Information & Collected information: credentials, network information, hostname, username, specific files of interest, documents, screenshots (38) \\
% %     System abuse & Protocol: HTTP/S, DropBox API, DNS, Mail, ADFS server, Exchange web service, outlook (22) \\
% %     Malicious object & Webshell, file stealer (3) \\ 
% %     \bottomrule \\ 
% %     \caption{How techniques are implemented}
% %     \label{tab:procedureCodes}
% % \end{longtable}
% % \end{scriptsize}

% Cyberattackers use a plethora of techniques depending on the attack types (e.g., data breach, denial of service) and victim environment (e.g., personal computer, cloud). Malware databases, cyberthreat encyclopedias,~\cite{kasperskythreatencyclopedia, trendmicrothreatencyclopedia} and CTI reports document adversarial techniques in their descriptions of how an attack unfolded or how a particular malware worked. 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \scriptsize
% \caption{Summary of the evaluation of our findings against a set of unseen CTI reports}
% \label{tab:evaluation}
% \begin{tabular}{lr}
% \toprule
% \textbf{Evaluation   measures}                            & \textbf{Value} \\ \midrule
% Number of attack instances                                & 125            \\
% Mean (median) count of reported techniques per   instance          & 12.86 (11)          \\
% Count of unique techniques across all   instances         & 333            \\
% Count of common unique techniques across   all instances and identified pairs & 144 \\
% Prevalent techniques found                                & 17             \\
% Mean (median) count of found prevalent techniques   per instance   & 2.66 (2)           \\
% Count of   valid pairs                             & 317            \\
% Count of   valid pairs found across all instances  & 228            \\
% Count of   instances where at least one valid pair is found                   & 86  \\
% Mean (median)  count of valid pairs found per instance     & 5.86 (2)          \\
% \bottomrule
% \end{tabular}%
% \end{table}

==> garbage/notes.tex <==
\begin{itemize}
    \item characterization of malicious software used in APT attacks
    \item two aspects
    \begin{itemize}
        \item what techniques these malware used
        \item what techniques are related
        \item what are the malware behavior and how are they connected
        \item what are the behavior associated with the malware, such as how are they distributed
        \item what are the takeaways for software developers
        \begin{itemize}
            \item focus on the fact that security is an afterthought - software development process should acknowledge how adversarial techniques are used, or even how their benign software- such as, Dropbox - can be turned into malicious ones 
            \item vulnerabilities
            \item abuse of their APIs
            \item permission required for apparently reading operations, such as systeminfo
            \item shared modules related issues, they should be bundled as an appImage
            \item authorized install-able channels, so that users do not get tempted by phishing emails
            \item introduce passwordless authentications in every software
            \item OS developers needs to address startup/registry/task related issues, which can really be abused easily
        \end{itemize}
    \end{itemize}
    \item 
\end{itemize}
